Using a Feedback Loop for LLM-based Infrastructure as Code Generation

Code generation with Large Language Models (LLMs) has helped to increase software developer productivity in coding tasks, but has yet to have significant impact on the tasks of software developers that surround this code. In particular, the challenge of infrastructure management remains an open question. We investigate the ability of an LLM agent to construct infrastructure using the Infrastructure as Code (IaC) paradigm. We particularly investigate the use of a feedback loop that returns errors and warnings on the generated IaC to allow the LLM agent to improve the code. We find that, for each iteration of the loop, its effectiveness decreases exponentially until it plateaus at a certain point and becomes ineffective.

==> sections/correctnessDefs.tex <==
\section{Notions of Correctness}



\subsection{Semantic}
A schema validator is able to check a number of the defined semantic properties:
\begin{enumerate}
    \item A set of keywords
    \item The relative positional correctness of these keywords
    \item Types of the values for each keyword. 
    \item type error that require recursive type checking (see below)
    \item any other issue that would be a compile time error
\end{enumerate}
As a note, JSON schema definition provided by [\url{}] allows for extended type systems, which could check properties such as a regular expression on a string (e.g. IP address). We restrict this type of checking to non-recursive type checking, i.e., type checking a value that does not require type look up of subvalues.



%g :: Int -> Int
%f :: Int -> Int -> Int
%x :: String
%{f : "+", x: "hello", g : "f x"}

Additionally, runtime errors are in the category of semantic correctness.
However, in practice these are not errors that can be encoded into a JSON schema.
In order to encode runtime errors into a JSON schema, the runtime system of the computational language represented by the JSON object would need to be encoded into the JSON schema.
If achieved, such errors would now be checked at compile time and thus become compile time errors.
% def schema
% run https://github.com/networknt/json-schema-validator?tab=readme-ov-file
% TODO look into output (number of validation errors?)
% example of schema (in)correctnes

\subsection{Conceptual}
%The notion of conceptual correctness, as distinct from semantic correctness, is that the generated JSON conceptually matches the specification (natural language prompt). Because the specification is given in natural language in the case of an LLM, this is an inherently informally defined notion of correctness.

We consider conceptual correctness, as distinct from semantic correctness, to be the conceptual match between the generated JSON and the specification. Since, in the case of an LLM, the specification is given in natural language, this measure is inherently informal. 

% def 
% https://github.com/aws-cloudformation/cfn-lint?tab=readme-ov-file
% example of semantic (in)correctnes

% def conceptual
% example of conceptual (in)correctnes

\section{Our Tool}
